Evaluating Biomedical BERT Models for Vocabulary Alignment at Scale in the UMLS Metathesaurus

The current UMLS (Unified Medical Language System) Metathesaurus construction process for integrating over 200 biomedical source vocabularies is expensive and error-prone as it relies on the lexical algorithms and human editors for deciding if the two biomedical terms are synonymous. Recent advances in Natural Language Processing such as Transformer models like BERT and its biomedical variants with contextualized word embeddings have achieved state-of-the-art (SOTA) performance on downstream tasks. We aim to validate if these approaches using the BERT models can actually outperform the existing approaches for predicting synonymy in the UMLS Metathesaurus. In the existing Siamese Networks with LSTM and BioWordVec embeddings, we replace the BioWordVec embeddings with the biomedical BERT embeddings extracted from each BERT model using different ways of extraction. In the Transformer architecture, we evaluate the use of the different biomedical BERT models that have been pre-trained using different datasets and tasks. Given the SOTA performance of these BERT models for other downstream tasks, our experiments yield surprisingly interesting results: (1) in both model architectures, the approaches employing these biomedical BERT-based models do not outperform the existing approaches using Siamese Network with BioWordVec embeddings for the UMLS synonymy prediction task, (2) the original BioBERT large model that has not been pre-trained with the UMLS outperforms the SapBERT models that have been pre-trained with the UMLS, and (3) using the Siamese Networks yields better performance for synonymy prediction when compared to using the biomedical BERT models.

==> back_up_text.tex <==
Table \ref{example_triples} contains examples of synonymous atoms and the various types of identifiers assigned to each respective atom for a particular concept (i.e. C0018681). Each atom is a term from a specific source vocabulary and each concept is a cluster (or grouping) of atoms. All atoms in the UMLS Metathesaurus are assigned a unique identifier (AUI) and a source concept identifier (SCUI) that indicates the source vocabulary the atom is introduced from. Every occurrence of a term in each source vocabulary is also assigned a unique atom identifier (AUI). When the same term appears in various source vocabularies, for example, “Cephalodynia” appearing in both MSH and SNOMEDCT\_US, they are assigned different AUIs “A26628141” and “A2957278” as shown in Table \ref{example_triples}. 

% \begin{table}
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{|l|l|l|l|l|}
% \hline
% Tuple & String & Source & AUI & CUI \\ \hline
% $t_1$ & Headache & MSH & A0066000 & C0018681 \\ \hline
% $t_2$ & Headaches & MSH & A0066008 & C0018681 \\ \hline
% $t_3$ & Cranial Pains & MSH & A1641924  & C0018681   \\ \hline
% $t_4$ & Cephalodynia & MSH & A26628141 & C0018681  \\ \hline
% $t_5$ & Cephalodynia & SNOMEDCT\_US & A2957278 & C0018681  \\ \hline
% $t_6$ & Headache (finding) & SNOMEDCT\_US & A3487586 & C0018681 \\ \hline
% \end{tabular}
% }

Given the success of transformer models for different NLP tasks, the objective of this work is to investigate the performance of context-aware embeddings extracted using different methods from various domain-specific BERT models with the Siamese networks introduced in \cite{nguyenadding, nguyen2021biomedical}. Additionally, we use the same pre-trained BERT models and adapt them for the UVA task. Section \ref{approach} contains the experimental details for the respective objectives. 

\textbf{Contributions.} Quite surprisingly, our results indicate that the Siamese networks initialized with embeddings extracted from off-the-self BERT models do not outperform the networks initialized with BioWordVec embeddings. Additionally, we find that pre-trained domain-specific BERT models do not outperform the Siamese Network for the UVA. \textcolor{red}{Our results indicate that fine-tuning the BERT embeddings with the domain specific task leads to better performance. 
Through our extensive feature extraction experiments, we find that using average token embeddings leads to better performance than first and last embeddings. Moreover using the average of the embeddings extracted from the last four layers of the BERT model also increases the performance the downstream task.} 

The construction process receives tuples from the UMLS Metathesaurus as input. The tuples shown here consist of ($str$, $src$, $aui$, $cui$), where $str$ is the original string of the term from the source vocabulary ($src$), $aui$ is the unique atom identifier, and $cui$ is the unique concept identifier.
%, and $scui$ is the unique identifier of that $str$ string from the source vocabulary. 
Let $T$ $=$ $(S_{STR}, S_{SRC}, S_{AUI}, S_{CUI})$ be the set of all input tuples in the Metathesaurus where:

$S_{STR}$ is the set of all atom names, 

$S_{SRC}$ is the set of all source vocabulary names, 

$S_{SCUI}$ is the set of all source concept unique identifiers,

$S_{AUI}$ is the set of all atom unique identifiers, and

% $S_{CUI}$ is the set of all concept unique identifiers. 

The Metathesaurus is a growing system that consists of approximately 10 million English atoms, each of which is associated with one of the 4.28 million concepts and is updated every six months. During the construction process, each AUI is assigned a single concept. 

The Metathesaurus integration process is given input tuple pairs ($t_i$, $t_j$), where $i \neq j$, in the form of ($str$, $src$, $aui$, $cui$), as instances of $T$, the set of all atom pairs, initialized from the different source vocabularies using the different identifier types for characterizing atoms as described above.

% Recent advances in Natural Language Processing (NLP) have led to better performing contexualized embeddings that are learned using Transformer models (e.g. BERT) \cite{devlin2018bert}. Transformer models generate context-aware embeddings that outperform traditional word embeddings like  word2vec \cite{mikolov2013distributed}, fastText \cite{bojanowski2017enriching}, and Glove \cite{pennington2014glove} on different downstream tasks. Embeddings extracted from models like word2vec, fastText, and Glove have a fixed representation for each word regardless of the context within which the word appears. However, BERT produces contextualized word representations that are informed by the surrounding words in the input. Embeddings extracted from BERT models have outperformed Word2Vec based embeddings on several NLP tasks \cite{devlin2018bert}. In Section \ref{related_work}, we provide more details about the different Transformer models used in our work. 

The tuples shown here consist of ($str$, $src$, $scui$, $aui$, $cui$), where $str$ is the original string from the source vocabulary ($src$), and $scui$ is the unique identifier of that $str$ string from the source vocabulary. 
Let $T$ $=$ $(S_{STR}, S_{SRC}, S_{SCUI}, S_{AUI}, S_{CUI})$ be the set of all input tuples in the Metathesaurus where:









 The Metathesaurus integration process is given input tuple pairs ($t_i$, $t_j$), where $i \neq j$, in the form of ($str$, $src$, $scui$, $cui$), as instances of T initialized from the different source vocabularies using the several identifier types for characterizing atoms as described above.
Given a set of tuples, $T$, as input from source vocabularies, the goal for the synonym prediction task to measure the similarity among atoms in a tuple. Let $T$ be a set of all input tuples in the form of ($(S_{STR}, S_{SRC}, S_{AUI}, S_{CUI})$), where:

$S_{STR}$ is the set of all atom names, 
$S_{SRC}$ is the set of all source vocabulary names, 
$S_{AUI}$ is the set of all atom unique identifiers, and
$S_{CUI}$ is the set of all concept unique identifiers. 
The tuples $t_1$, $t_3$, $t_4$, and $t_5$ are all instances of $T$.


% \textit{*Introduce only the notion we use in our paper, just wondering if we are using SCUI in our experiments?*}

% \begin{table}[]
% \begin{center}
% %\resizebox{\columnwidth}{!}{
% \begin{tabular}{|l|l|l|}
% \hline
% Notion & Meaning \\ \hline
% $SRC$ & Vocabulary source \\ \hline 
% $T$ & set of tuples  \\ \hline
% $STR$ & Atom string \\ \hline
% $AUI$ & Atom unique ID \\ \hline
% $CUI$ & Concept unique ID  \\ \hline
% $SCUI$ & Source CUI  \\ \hline
% \end{tabular}
% %}
% \end{center}
% \caption{}
% \label{notions_meanings}
% \end{table}


%\sout{that links terms and codes between health records, pharmacy documents, and insurance documents, enabling interoperability among them} \cite{bodenreider2004unified}. 

% The synonymy prediction task decides if the atoms in each input tuple pair are synonymous. Nguyen et al. \cite{nguyen2021biomedical} assess the similarity of atoms using lexical features of the atom strings ($src$). 
% They design a Siamese Netowrk that uses a pair of atom strings as input, ($src_i, src_j$), where  $i \neq j$, and outputs a similarity score between 0 and 1, $sim{(src_i, src_j)} \in [0, 1]$. The model then encodes each atom and compares the output representation using a distance metric (i.e. Manhattan distance) to measure similarity. The higher the similarity (or the lower the distance) between the two atoms in a pair the more likely these atoms are to be synonymous. This problem setup allows for a more computationally feasible method (when compared to classification approaches) to identify synonymous for new atoms that are introduced during the UMLS Metathesaurus updates every six months.
